Robust 6D Object Pose Estimation with Stochastic Congruent Sets

Object pose estimation is frequently achieved by first segmenting an RGB image and then, given depth data, registering the corresponding point cloud segment against the object's 3D model. Despite the progress due to CNNs, semantic segmentation output can be noisy, especially when the CNN is only trained on synthetic data. This causes registration methods to fail in estimating a good object pose. This work proposes a novel stochastic optimization process that treats the segmentation output of CNNs as a confidence probability. The algorithm, called Stochastic Congruent Sets (StoCS), samples pointsets on the point cloud according to the soft segmentation distribution and so as to agree with the object's known geometry. The pointsets are then matched to congruent sets on the 3D object model to generate pose estimates. StoCS is shown to be robust on an APC dataset, despite the fact the CNN is trained only on synthetic data. In the YCB dataset, StoCS outperforms a recent network for 6D pose estimation and alternative pointset matching techniques.

==> super4pcs.tex <==
\SetKwProg{Fn}{Function}{}{}

\begin{algorithm}[h]
\label{alg:alg2}
\caption{{\sc SUPER4PCS}( {\tt S}, {\tt M}, {$\delta$}) }
\Fn{{\sc compute\_best\_transform (S, M, $\delta$)}}{
	bestScore $\gets$ 0 \;
	$T_{opt}$ $\gets$ identity transform \;
	\For{iter = 1:max\_iterations}{
		B $\gets$ {\sc select\_coplanar\_base(S, M)}\;
		U $\gets$ {\sc find\_congruent\_set(B, M)}\;
	
		\ForEach{4-point set $U_i$ $\in$ U}{
			$T_i$ $\gets$ best rigid transform that aligns B to $U_i$ in the least square sense\;
			Find $S_i \subset P$, such that $d(T(S_i),Q) < \delta$\;
		}
		k $\gets$ $argmax_i$ {$\mid S_i \mid$} \;
		\If{{$\mid S_k \mid$} $>$ bestScore}{
			bestScore $\gets$ $\mid S_k \mid$ \;
			$T_{opt}$ $\gets$ $T_k$ \;
		}
	}
	return $T_{opt}$\;
}
\BlankLine
\Fn{{\sc select\_coplanar\_base (S, M)}}{
	$b_1$ $\gets$ random\_sample(S) \;
	max\_angle $\gets$ 0 \;
	\For{$iter = 1:max\_trials$}{
		$b_2$ $\gets$ random\_sample(S) \;
		$b_3$ $\gets$ random\_sample(S) \;
		\If{angle($b_2$, $b_3$) $>$ max\_angle $\And \mid b_1 - b_2 \mid  < $ diameter(M) $\And \mid b_1 - b_3 \mid  < $ diameter(M)}{
			update $b_2$, $b_3$ \;
		}
	}

	best\_plane\_distance $\gets$ intmax \;

	\For{$i = 1:\mid S \mid$}{
		\If{$\mid S_i - b_1 \mid  > $ 0.2*diameter(M) $\And \mid S_i - b_2 \mid  > $ 0.2*diameter(M) $\And \mid S_i - b_3 \mid  > $ 0.2*diameter(M)}{
			plane\_distance $\gets$ dist(plane($b_1,b_2,b_3$), $S_i$)\;
			\If{plane\_distance $<$ best\_plane\_distance}{
				accept $S_i$ \;
				best\_plane\_distance $\gets$ plane\_distance \;
			}
		}
	}
	return $b_1, b_2, b_3, b_4$\;
}
\BlankLine
\Fn{{\sc find\_congruent\_set(B, M, $\delta$)}}{
	$d_1$ $\gets$ $\mid\mid b_1 - b_2 \mid\mid$ \;
	$d_2$ $\gets$ $\mid\mid b_3 - b_4 \mid\mid$ \;
	compute $R_1$ = {($P_i,P_j \mid P_i,P_j \in M$)}, $\mid\mid P_i - P_j \mid\mid \in [d_1 - \delta, d_1 + \delta]$ \;
	compute $R_2$ = {($P_i,P_j \mid P_i,P_j \in M$)}, $\mid\mid P_i - P_j \mid\mid \in [d_2 - \delta, d_2 + \delta]$ \;
	\ForEach{$r_{1i} \in R_1$}{
		Compute the 4 points, {$e_{1i}^1, e_{1i}^2, e_{1i}^3, e_{1i}^4$} related to the invariants $r_1, r_2$ \;
	}
	Build an approximate range tree structure for the point set $e_{1i}^j$ \;
	\ForEach{$r_{2i} \in R_2$}{
		Compute the 4 points, {$e_{2i}^1, e_{2i}^2, e_{2i}^3, e_{2i}^4$} related to the invariants $r_1, r_2$ \;
	}
	\ForEach{$e_{2i}^j$}{
		Using RS, retrieve all points in $\delta$-neighborhood of query point $e_{1i}^j$. For each such point q, create candidate 4-points sets corresponding to B as U \;
	}
	return U \;
}
\end{algorithm}

